Calibration of the charge and energy loss per unit length of the MicroBooNE liquid argon time projection chamber using muons and protons

We describe a method used to calibrate the position- and time-dependent response of the MicroBooNE liquid argon time projection chamber anode wires to ionization particle energy loss. The method makes use of crossing cosmic-ray muons to partially correct anode wire signals for multiple effects as a function of time and position, including cross-connected TPC wires, space charge effects, electron attachment to impurities, diffusion, and recombination. The overall energy scale is then determined using fully-contained beam-induced muons originating and stopping in the active region of the detector. Using this method, we obtain an absolute energy scale uncertainty of 2\% in data. We use stopping protons to further refine the relation between the measured charge and the energy loss for highly-ionizing particles. This data-driven detector calibration improves both the measurement of total deposited energy and particle identification based on energy loss per unit length as a function of residual range. As an example, the proton selection efficiency is increased by 2\% after detector calibration.

==> saved/old_ana_met_dqdx.tex <==
% % This is subsection 2.4 as it was as of
% %  Thu Oct 3 21:41:50 2019 +0000 (16:41:50 CDT)
% % before major rewrite by Glenn.

\subsection{Analysis method}
\label{sec:ana_met_dqdx}
The $dQ/dx$ calibration of the detector is carried out in three separate steps for the collection plane.
\begin{itemize}
\item Step 1: Detector calibration in the yz plane. This step aims to remove the effects of space charge, misconfigured or cross-connected anode plane channels, and transverse diffusion.
\item Step 2: Detector calibration in the drift (x) direction. This step removes effects of electron attenuation, space charge, and longitudinal diffusion.
\item Step 3: Detector calibration in time. This step aims to remove any temporal variations in the detector response. This step is only performed for data. There is currently no time dependence in the MC simulation.
\end{itemize}

\subsubsection{Procedure for detector calibration in the yz plane}
\label{sec:yz_cal}
 Once we have a sample consisting of anode-cathode crossing CR tracks, we use the following procedure to determine the $dQ/dx$ calibration in the yz plane:

\begin{enumerate}[label=(\roman*)]     

\item Isolate crossing CR tracks identified by the selection in section~\ref{sec:sel_cut_rel}.

\item Calculate staring time ($t_{0}$); for crossing CR the minimum drift coordinate corresponds to $t_{0}$ times the ionization drift velocity.

\item Calculate the drift coordinate $x_\textit{Corrected}$ of each three-dimensional (3D) space point on the track using the $t_{0}$ (i.e., $x_\textit{Corrected}$ = $x_\textit{Uncorrected}$ - $\textit{drift velocity}~\times~t_\textit{0}$).

\item Segment the yz plane into 5 cm by 5 cm cells.

%\item Group each 3D point into its relevant cell in yz using the $y$ and $z$ coordinates that satisfy the conditions 0 cm $<$ $x_\textit{Corrected}$ $<$ 260 cm, -120 cm $< y <$ 120 cm, and 0 cm $< z <$ 1040 cm.

\item Group each 3D point into its relevant cell in yz using the $y$ and $z$ coordinates that are completely within TPC boundaries defined in figure~\ref{fig:theta_xz_yz_def}.

\item After looping over all crossing CR tracks, only keep cells which have at least five 3D track points.

\item For each of the selected cells, we calculate a median $dQ/dx$ value by considering charge information of all the 3D points in that cell. The median $dQ/dx$ of a given cell is called the \say{local median $dQ/dx$} of that cell (median $dQ/dx$ is chosen to remove delta ray contamination and misreconstructed calorimetric information).

\item Calculate the \say{global median dQ/dx} by taking the median $dQ/dx$ value from all the 3D points coming from all crossing tracks. This median is taken over all non-empty cells as well.

\item For each cell in the yz plane, define a correction factor $C(y_{i},z_{i})$ using; 
\end{enumerate}

\begin{equation}
\label{eqn:cor_fact_yz}
C(y_{i},z_{i}) = \frac{(dQ/dx)_{Global}}{((dQ/dx)(y_{i},z_{i}))_{Local}}\,.
\end{equation}

\subsubsection{Procedure for detector calibration in the drift direction}
\label{sec:x_cal}

After calibrating the yz plane, we next move to the drift direction calibration of the detector. The following explains how this calibration procedure is carried out:

\begin{enumerate}[label=(\roman*)]

\item Isolate crossing CR tracks and calculate the drift coordinate $x_\textit{Corrected}$ of each three-dimensional (3D) space point on tracks as in the procedure for yz plane calibration.

\item Correct the charge information ($dQ/dx$) of each 3D point using yz correction factors, derived in the previous step, to remove the irregularities in the yz plane using equation~\ref{eqn:yz_corrected}. If cells do not have a minimum of five 3D track points, yz correction factors of nearby cells are used to correct the charge information. Here we select the 3D points that are within TPC boundaries.
%Here we select the 3D points that satisfy \newline 
%0 cm $<$ $x_\textit{Corrected}$ $<$ 260 cm, -120 cm $< y <$ 120 cm, and 0 cm $< z <$ 1040 cm. 
Moreover we examine the $y$ and $z$ coordinates of the 3D point to determine which yz correction factor to use.

\begin{equation}
\label{eqn:yz_corrected}
((dQ/dx)(y_{i},z_{i}))_{Corrected} = C(y_{i},z_{i})\cdot((dQ/dx)(y_{i},z_{i}))_{Reconstructed}~,
\end{equation}

where $((dQ/dx)(y_{i},z_{i}))_{Corrected}$ is the corrected $(dQ/dx)$ value by $C(y_{i},z_{i})$ correction factor for irregularities in the yz plane, and  $((dQ/dx)(y_{i},z_{i}))_{Reconstructed}$ is the uncorrected $dQ/dx$ value.

\end{enumerate}

\begin{enumerate}[label=(\roman*)]
\setcounter{enumi}{3}

\item Segment the drift direction into bins of 10 cm in data and bins of 5 cm in MC. Bin sizes are chosen to minimize statistical fluctuations in the correction factors.

\item Group each 3D point into the relevant drift direction bin based on its corrected $x$ coordinate.

\item Define a \say{local median $dQ/dx$} for each of the bins in the drift direction which has more than five 3D points.

\item Define \say{global median $dQ/dx$} as explained in the previous calibration procedure.

\item for each bin in the drift direction, a correction factor $C(x_{i})$ is defined using equation~\ref{eqn:cor_fact_x};

\begin{equation}
\label{eqn:cor_fact_x}
C(x_{i}) = \frac{(dQ/dx)^{\prime}_{Global}}{((dQ/dx)(x_{i}))^{\prime}_{Local}}~,
\end{equation}

where $(dQ/dx)^{\prime}_{Global}$ is the global median $dQ/dx$ value after correcting for yz plane irregularities by equation~\ref{eqn:yz_corrected} in the collection plane, and $((dQ/dx)(x_{i}))^{\prime}_{Local}$ is the local $dQ/dx$ median for the given $x_{i}$ position after correcting for yz plane irregularities by equation~\ref{eqn:yz_corrected} in the collection plane.

\end{enumerate}

In data, we derive the drift direction correction factors for each day as space charge effects and electron lifetime can change over time. To get a reliable set of correction factors, we need a data sample which contains enough statistics. For this purpose, we derive correction factors in the drift direction only for the days where there are more than 40 crossing tracks after all the angular cuts. In the case of lack of statistics for a given day, we use the drift direction correction factors derived for the immediate neighboring day. For MC we derive only a single set of drift direction correction factors for the collection plane as there is no time variation of space charge effects and electron attenuation. 

\subsubsection{Procedure for time dependent calibration of the detector}
\label{sec:t_cal}

Next, temporal variations in the detector response are addressed. The following set of steps explains how the detector calibration in time is achieved:

\begin{enumerate}[label=(\roman*)]

\item Select tracks and hits as described in sections~\ref{sec:yz_cal} and~\ref{sec:x_cal}.

\item Correct $dQ/dx$ value of each 3D track point using correction factors derived for the yz plane and drift direction using equation~\ref{eqn:xyz_corrected} for the reconstructed $x$, $y$, and $z$ coordinates.

\begin{equation}
\label{eqn:xyz_corrected}
((dQ/dx)(x_{i},y_{i},z_{i}))_{Corrected} = C(y_{i},z_{i}) \cdot C(x_{i}) \cdot ((dQ/dx)(x_{i},y_{i},z_{i}))_{Reconstructed}~,
\end{equation}

where $((dQ/dx)(x_{i},y_{i},z_{i}))_{Corrected}$ is the corrected $dQ/dx$ value for yz plane and drift direction irregularities in the collection plane, and $((dQ/dx)(x_{i},y_{i},z_{i}))_{Reconstructed}$ is the uncorrected $dQ/dx$ value in the collection plane.

\item Calculate a \say{global median $dQ/dx$} value by taking the median $dQ/dx$ value of all the hits in the entire TPC volume for the day, we want. In the time calibration of the detector, we calculate this global median $dQ/dx$ value on a daily basis.

\item Plot the global median $dQ/dx$ values against time to visualize the detector variations in time (See figure~\ref{fig:time_corre_gbl_mdn}).

\item Choose the reference value (210 ADC/cm) for the global median $dQ/dx$ in the collection plane, since all global median $dQ/dx$ values calculated for each day fluctuate around this value. See figure~\ref{fig:time_corre_gbl_mdn}.

\item Determine a time dependent correction $C(t)$ using equation~\ref{eqn:time_cor} for each day. 

%\begin{equation}
%\label{eqn:xyz_corrected}
%((dQ/dx)(x_{i},y_{i},z_{i}))_{Corrected} = C(y_{i},z_{i}) \cdot C(x_{i}) %\cdot ((dQ/dx)(x_{i},y_{i},z_{i}))_{Reconstructed}~,
%\end{equation}

%where $((dQ/dx)(x_{i},y_{i},z_{i}))_{Corrected}$ is the corrected $dQ/dx$ value for yz plane and drift direction irregularities in the collection plane, and $((dQ/dx)(x_{i},y_{i},z_{i}))_{Reconstructed}$ is the uncorrected $dQ/dx$ value in the collection plane.

\begin{equation}
\label{eqn:time_cor}
C(t) = \frac{(dQ/dx)_{Reference}}{((dQ/dx)(t))_{Global}}~,
\end{equation}

where $(dQ/dx)_{Reference}$ is the reference $dQ/dx$ value in the collection plane, and\newline $((dQ/dx)(t))_{Global}$ is the global $dQ/dx$ value in the collection plane after correcting for yz plane and drift direction irregularities for each day.
\end{enumerate}

\begin{figure}[!ht]
\centering

\includegraphics[width=0.49\textwidth]{figures/Fig_18_L_edit5.pdf}
\includegraphics[width=0.49\textwidth]{figures/run3/run3_dqdxMedian_time.pdf}
\caption{The global median $dQ/dx$ per day over time in the collection plane. The red lines drawn shows the reference value selected which is 210 ADC/cm. Left: the global median $dQ/dx$ from February 10, 2016 to October 17, 2016 in run period \rom{1}. Right: the global median $dQ/dx$ from October 27, 2017 to March 16, 2018 in run period \rom{3}. Dips from the reference values across several days are due to time periods in which argon purity was low (e.g. during recirculation pump maintenance). }

\label{fig:time_corre_gbl_mdn}
\end{figure}

Once we are finished with calibrating the detector in the yz plane, drift direction, and in time, we can use equation~\ref{eqn:cor_dqdx_data} and equation~\ref{eqn:cor_dqdx_mc} to compute the calibrated $dQ/dx$ values in data and MC, respectively.

\begin{equation}
\label{eqn:cor_dqdx_data}
((dQ/dx)(x_{i},y_{i},z_{i},t))_{Corrected}^{data} = ((dQ/dx)(x_{i},y_{i},z_{i},t))_{Reconstructed}\cdot C(y_{i},z_{i}) \cdot C(x_{i}) \cdot C(t)~,
\end{equation}

where $((dQ/dx)(x_{i},y_{i},z_{i},t))_{Corrected}^{data}$ is the corrected $dQ/dx$ for yz plane, drift direction irregularities and time variations in data in the collection plane, and $((dQ/dx)(x_{i},y_{i},z_{i},t))_{Reconstructed}$ is the uncorrected $dQ/dx$ in data in the collection plane.

\begin{equation}
\label{eqn:cor_dqdx_mc}
((dQ/dx)(x_{i},y_{i},z_{i}))_{Corrected}^{MC} = ((dQ/dx)(x_{i},y_{i},z_{i}))_{Reconstructed}\cdot C(y_{i},z_{i}) \cdot C(x_{i})~,
\end{equation}

where $((dQ/dx)(x_{i},y_{i},z_{i}))_{Corrected}^{MC}$ is the corrected $dQ/dx$ for yz plane and drift direction irregularities in MC in the collection plane, and $((dQ/dx)(x_{i},y_{i},z_{i}))_{Reconstructed}$ uncorrected $dQ/dx$ in MC in the collection plane.


